ACTRESS: Active Retraining for Semi-supervised Visual Grounding

Semi-Supervised Visual Grounding (SSVG) is a new challenge for its sparse labeled data with the need for multimodel understanding. A previous study, RefTeacher, makes the first attempt to tackle this task by adopting the teacher-student framework to provide pseudo confidence supervision and attention-based supervision. However, this approach is incompatible with current state-of-the-art visual grounding models, which follow the Transformer-based pipeline. These pipelines directly regress results without region proposals or foreground binary classification, rendering them unsuitable for fitting in RefTeacher due to the absence of confidence scores. Furthermore, the geometric difference in teacher and student inputs, stemming from different data augmentations, induces natural misalignment in attention-based constraints. To establish a compatible SSVG framework, our paper proposes the ACTive REtraining approach for Semi-Supervised Visual Grounding, abbreviated as ACTRESS. Initially, the model is enhanced by incorporating an additional quantized detection head to expose its detection confidence. Building upon this, ACTRESS consists of an active sampling strategy and a selective retraining strategy. The active sampling strategy iteratively selects high-quality pseudo labels by evaluating three crucial aspects: Faithfulness, Robustness, and Confidence, optimizing the utilization of unlabeled data. The selective retraining strategy retrains the model with periodic re-initialization of specific parameters, facilitating the model's escape from local minima. Extensive experiments demonstrates our superior performance on widely-used benchmark datasets.

==> sec/draw.tex <==

\begin{figure*}[t]
\centering
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a clear mixing bowl full of chocolate mix_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a donut to the right of two other donuts_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a giraffe that has its face visible_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a gray and undetached train cart on the tracks_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a green vw van_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a knit bear figure to the right of a duplicate_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a man in a red shirt eating sweets with his friend_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/a round wall clock showing london time next to two other clocks showing times for other cities_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/brown dog_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/good_case/chocolate dessert cake on a plate_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/bad_case/a boat_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/bad_case/a laptop with a blank screen_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/bad_case/a traveler with a black and yellow bag on his bag with others on transit_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/bad_case/apple furthest to the right_.pdf}
\end{minipage}
\begin{minipage}{0.17\textwidth}
\centering
\includegraphics[width=0.94\textwidth]{sec/bad_case/stuffed teddy bear with a red ribbon_.pdf}
\end{minipage}
\end{figure*}
